Generating Context-Aware Natural Answers for Questions in 3D Scenes

3D question answering is a young field in 3D vision-language that is yet to be explored. Previous methods are limited to a pre-defined answer space and cannot generate answers naturally. In this work, we pivot the question answering task to a sequence generation task to generate free-form natural answers for questions in 3D scenes (Gen3DQA). To this end, we optimize our model directly on the language rewards to secure the global sentence semantics. Here, we also adapt a pragmatic language understanding reward to further improve the sentence quality. Our method sets a new SOTA on the ScanQA benchmark (CIDEr score 72.22/66.57 on the test sets).

==> sections/title.tex <==
\title{Question Generation for Question Answering in 3D Scenes}

% Enter the paper's authors in order
% \addauthor{Name}{email/homepage}{INSTITUTION_CODE}
\addauthor{Mohammed Munzer Dwedari}{munzer.dwedaru@tum.de}{1}

% Enter the institutions
% \addinstitution{Name\\Address}
\addinstitution{
 Visual Computing and Artificial Intelligence Lab\\
 Technical University of Munich\\
 Munich, Germany
}
